PointWise: An Unsupervised Point-wise Feature Learning Network

We present a novel approach to learning a point-wise, meaningful embedding for point-clouds in an unsupervised manner, through the use of neural-networks. The domain of point-cloud processing via neural-networks is rapidly evolving, with novel architectures and applications frequently emerging. Within this field of research, the availability and plethora of unlabeled point-clouds as well as their possible applications make finding ways of characterizing this type of data appealing. Though significant advancement was achieved in the realm of unsupervised learning, its adaptation to the point-cloud representation is not trivial. Previous research focuses on the embedding of entire point-clouds representing an object in a meaningful manner. We present a deep learning framework to learn point-wise description from a set of shapes without supervision. Our approach leverages self-supervision to define a relevant loss function to learn rich per-point features. We train a neural-network with objectives based on context derived directly from the raw data, with no added annotation. We use local structures of point-clouds to incorporate geometric information into each point's latent representation. In addition to using local geometric information, we encourage adjacent points to have similar representations and vice-versa, creating a smoother, more descriptive representation. We demonstrate the ability of our method to capture meaningful point-wise features through three applications. By clustering the learned embedding space, we perform unsupervised part-segmentation on point clouds. By calculating euclidean distance in the latent space we derive semantic point-analogies. Finally, by retrieving nearest-neighbors in our learned latent space we present meaningful point-correspondence within and among point-clouds.

==> figures/teaser.tex <==
%\begin{teaserfigure}
%\includegraphics[width=\columnwidth]{figures/Teaser_6.png}
%\caption{Write caption
%}
%\label{fig:teaser}
%\end{teaserfigure}

==> method_old.tex <==
\section{METHOD}

%Let us define some key notations: We shall denote a given point-cloud as \({C_i}\) and the points comprising it as \(\left\{p_{i,j} : j=1,...,N\right\}\). The latent-space descriptor of the point \(p_{i,j}\) will be denoted by  \(f_{i,j}\). The set of all latent-space descriptors for the points in \(C_i\) will be denoted as \(F_i\).  We shall annotate the function applied by the network on a single point as $h\left(p\right)$, so that \(f_{i,j}=h\left(p_{i,j}\right)\). 

Given a point-cloud \({C_i}\) comprised of points \(\left\{p_{i,j} : j=1,...,N\right\}\), we denote the latent-space descriptor of the point \(p_{i,j}\) with  \(f_{i,j}\). The set of all latent-space descriptors for the points in \(C_i\) is denoted as \(F_i\).  Let $h$ denote the function that maps a single point $p$ to its associated descriptor: \(f_{i,j}=h\left(p_{i,j}\right)\). and finally, let $H$ denote the mapping of an entire point set to it's set of point-wise descriptors: \(F_{i}=H\left(C_{i}\right)\).

\dc{I break the text into subsections, but that is just temporarily}

\subsection{The concept}

\sharon{In order to achieve a feature representation which has a contextual meaning, the network has to be trained both on the content of the entire point-cloud and on features which refer to local properties of each point. Therefore, the network receives an entire point cloud (i.e. \({C_i}\)) as input - and outputs a set of point-wise feature vectors (i.e. \({F_i}\)). Each point-wise feature is composed from a concatenation of the global feature and the point feature.} 
\matan{I think that's very PointNet-specific, maybe it'll be better to discuss that later}
%Our network architecture must to be such that receives a point-cloud as input (i.e. \({C_i}\)) - and outputs a set of point-wise feature vectors (i.e. \({F_i}\)). 

\dc{The above claims that we want to learn both local and global context... this we inherent from PointNet? then why it is good for our objective? it should be explained.}


In this paper, we use a modified, untrained version of the PointNet segmentation network as described in \cite{qi2017pointnet}. 
Our network architecture is illustrated in fig. \ref{fig:Architecture}. The principal difference being that our network is aimed at learning a semantically-meaningful latent space in an \textbf{unsupervised} manner. For that end, a new loss must be used, that does not rely on a given ground-truth.

\dc{The above should be already known from the Related Work. We should be more brief here, and just claim that we use the network layers (or whatever it can be called) from PointNet, and train the network in an unsupervised manner. At this point, here, we should refer to the architecture figure}
\matan{done (need to write a caption)}

\subsection{The key idea!!!!}

In order to produce a descriptive latent-space in an unsupervised manner, our architecture includes a sense  of  "self supervision" as a means to define a relevant loss. 

The chosen loss term should encourage the network to learn a semantically meaningful point-wise description.
We formulate a loss which  yields a latent space  that is geometrically-descriptive on one hand, and context-aware on the other. 


\dc{The network,or $H$ lift $p$ from 3D to 8D... As I see it, it could replicate the xyz and generate the normals abc, and add two redundant scalars. Then the losses could be minimal, no?
The triplet loss would be small, since the most significant bits are xyz. The MLP can easily reconstruct abc (the normal) etc...

There is nothing really in the losses that encourage learning what is a component, or whatever. The fact that we succeed to segment is not because we encouraged anything. We are doing a bit better than a clustering of xyzabc, right?

We should have some "insight" into our losses.
Maybe not now, but in after we have a preliminary version of the paper.

I was wondering whether we can add a little disentanglement to enforce the feature not to include xyz per se, and thus really learn something.

But I believe we need to encourage the feature to learn something non-local, somehow.}
\matan{Looking at the PCA expected variances, I think it's visible that there are more than 6 prominent dimensions. I used dropout on one of the final layers, I hope this helps prevent or at lease reduce this degeneration. I do believe some sort of reconstruction loss could yield better results, but this would require some work as distance measuring in point clouds is tricky }


\subsection{The losses}

Our loss consists of three main components:
\begin{equation} 
\label{eq:loss_function}
L = L_{triplet} + L_{normal} + L_{reg}\\ 
\end{equation}

\textbf{Triplet loss:} The first term is a triplet margin loss. For a given point-cloud descriptor set $F_i$ and an arbitrary integer $M$,  let \(R=\{r_m : m=1,...,M\}\) be a subset of randomly chosen reference points.  We then define two more subsets with respect to $R$: \(G=\{g_m : m=1,...,M\}\) is a set of positive examples, under some yet to be defined context. \(B=\{b_m : m=1,...,M\}\) is a set of negative ones. The triplet loss is defined as follows:
\begin{align}
\label{eq:triplet loss}
\begin{split}
&L_{triplet}=\frac{1}{M} \Sigma_{m=1}^{M}{max\left\{d\left(r_m,g_m\right)-d\left(r_m,b_m\right)+margin,0\right\}}\\
&where:  \space d\left(x,y\right)=\left\|x-y\right\|_p
\end{split}
\end{align}
This component brings point descriptors in the latent space closer together, or drives them further apart, depending on some predefined interaction between their corresponding coordinates in the spacial domain. The criteria we used in order to determine the interaction is "matual kNN": consider a given reference descriptor $r_m=f_{i,j}$. A  descriptor $f_{i,k}$ is considered a positive example if the point $p_{i,k}$ is among the k nearest-neighbors of the point $p_{i,j}$, and if the number of  overlapping members in both points' k nearest neighbors passes some pre-defined threshold.
\matan{not sure I'm being clear here}
\dc{The above is generic, the question is what is positive and what is negative!!! how exactly this is defined????}

\textbf{Normal estimation loss:} the second term is a normal estimation loss. Let $e\left(f_{i,j}\right)$  be a function applied to each descriptor by a shared MLP trained along with the entire network in order to estimate point normals using the calculated descriptors. The true normal at point  $p_{i,j}$ will be noted as \(Nor\left(p_{i,j}\right)\).  The Normal estimation loss is then defined as:
\begin{align}
\label{eq:triplet loss}
\begin{split}
&L_{normal}=\frac{1}{N} \Sigma_{j=1}^{N}\left\|e\left(f_{i,j}\right)-Nor\left(p_{i,j}\right)\right\|_p
\end{split}
\end{align}
By minimizing this component we encourage our learned descriptors to perform a semantically-meaningful task. \dc{really? why????}
A feature space that achieves this goal is less likely to encode only local coordinate-dependent information and so, every point's descriptor is prone to encode information regarding the point's environment. 

\dc{Ok, normal is a bit non-local... we need something stronger}
\textbf{Regularization loss:} the third term is a regularization loss:
\begin{align}
\label{eq:triplet loss}
\begin{split}
&L_{normal}=\frac{1}{N} \Sigma_{j=1}^{N}\left[\left\|\left\|f_{i,j}\right\|_2-1\right\|_p+VAR\left(\left\|f_{i,j}\right\|_2\right)\right]
\end{split}
\end{align}


\begin{figure*}[t]
\includegraphics[width=\textwidth]{figures/architecture.png}
\caption{Architecture (complete this)}
\label{fig:Architecture}
\end{figure*}





==> old_intro.tex <==
\section{Introduction}

\dc{drafting a new intro, it present more directly to the key contribution, hopefully}

Recently, point clouds are getting more attention as an effective 3D representation in the realm of neural networks. Point clouds are simple and provide a compact approximation of the underlying 3D shape. The use of point clouds, however, is technically challenging since  point clouds are irregular and unordered. Significant progress has been made in the field of direct-processing of point-clouds using neural networks, with architectures such as PointNet \cite{qi2017pointnet} and PoiNtnet++\cite{qi2017pointnet++} that uses global pooling operations that bypass the lack of order, or with an architecture that transforms the points into a canonical regular configuration that allows performing convolutions \cite{li2018pointcnn}. These networks are trained with supervision, yielding global task-specific features per point cloud \dc{or per shape would be clearer?}. 

In this paper, we present a network that learns Point-wise meaningful features with no supervision. Having generic meaningful pointwise features immediately allows clustering the points to achieve meaningful segmentation, or match points from several models to find correspondence and                         analogies among shapes. If the per point features constitute semantic meaning, so does the segmentation and correspondence.

The key challenge is to train a network to learn point-wise features without supervision. \dc{Unsupervised learning} allows using the large and ever growing training data that is not annotated. Moreover, learning highly-descriptive features without supervision leads to more generic features that can be used in various applications, rather than being task-specific.

Our approach leverages architectures which compute internal per-point features. The training is self-supervised, where the losses are derived from the data's geometry itself. We show that the point-wise features are highly-descriptive, and carry more meaningful information, than otherwise the bare coordinates themselves.
\dc{Here we should refer to our teaser...}

We demonstrate the competence of learned point-wise features with fundamental applications such as part segmentation...

\matan{Much more concise! What about some discussion on unsupervised learning? Keep that for the background?}

\dc{It is above, no? I highlighted it two paragraphs above.}


\section{Old intro}


\dc{I have many comments, but let's start with the first paragraph}

The use of three-dimensional (3D) representations is ever-growing  in applications such as computer-vision, augmented-reality, autonomous-driving and many more. In this realm, point-clouds are an efficient representation from a learning perspective. 

\dc{Let's distinguish between the advantages of point clouds in general and if and how they are attractive from "learning perspective". So write first their advantage in general, and then why they are attractive for learning. I think the reason is only because it is a sparse representation.}

They are compact, easy to manipulate and scale, and comprise the output of many modern 3D scanning devices.  

Though attractive to perform, the processing of point-clouds summons several prominent challenges. For example, coordinates given in point-cloud form are unordered. \dc{Remove:That is, a single given point-cloud consisting of \(N\) points can be represented by \(N!\) different permutations - all equally valid.} A network that utilizes point-cloud input must be invariant to point order.  Another noticeable challenge arises for the non-regular characteristic of the representation, which does not allow the definition of a regular convolution.

\dc{Now, regarding the second paragraph}

 Recently, much progress has been made in the field of direct-processing of point-clouds using neural networks. Architectures such as PointNet \cite{qi2017pointnet} and PoiNtnet++\cite{qi2017pointnet++} utilize the symmetric nature of pooling functions in order to tackle the challenging characteristics of point-clouds. These architectures present state of the art performance in cloud classification and segmentation. The optimization process towards performing these tasks employs large datasets of labeled examples. \dc{the following is not interesting for us, we must quickly tell that we want to learn Pointwise features!} This allows networks to learn highly-descriptive feature representation of their respective data. When semantically-meaningful information is encoded in such a representation, a plethora of advantages arises. Such an encoding enables the performance of basic editing through algebraic manipulation \dc{what is an algebraic manipulation?} . Some examples are interpolation and analogies. 
 
In particular, one might be interested in obtaining a meaningful feature representation of individual points comprising a point-cloud model.\dc{But why? this is a critical point!!! why do care having per point feature} Such representation holds the potential to enable high-resolution, scalable editing of 3D models \dc{really? why???}. It allows, for example, to cluster points within a given model to achieve meaningful segmentation on one hand, or match points from several models to find correspondence and analogies on the other hand. \dc{Let's then not say "for example", let's claim that this allows x and y.}

As large as labeled datasets may be, the vast majority of available data remains unlabeled and so, cannot be utilized for the tasks described above. In order to overcome this obstacle, one can utilize unsupervised learning. This strategy is meant to produce valuable information from data that does not include annotation. We attempt \dc{why attempt? that is what we do. Sound more assertive and confident} to utilize recent advancements in the field of direct-processing of point-clouds using neural-networks architectures, as well as the ever-growing amount of available data in order to produce useful semantic latent-space representations of individual points in relevant models. In our research we address the challenge of providing a “self-supervised” formulation for learning a meaningful representation of point-cloud data. 

\dc{Up to here! (for now)}

%We encourage the network to learn a more meaningful latent space by 
\sharon{We encourage the network to learn a more meaningful latent space by taking into account the relative positions of the points in space as well as geometrical properties of the data which combined create a semantically meaningful loss. To that end, we define }
 a loss based on several attributes: 1) A triplet loss demanding similarity between the latent representations of close points and non-similarity between the representations of distant points. 2) A loss based on point-normals estimation accuracy 3) A regularization loss aimed to normalize the feature space.

\sharon{We suggest a new architecture suitable to extracting global and point-wise unsupervised features which have a contextual meaning. We show results using the features learnt to perform segmentation on various datasets. Even though the network is trained in a completely unsupervised manner, we achieve comparable results to supervised methods.}
%Our goal is to develop a suitable architecture to perform this task, as well as to modify the existing method of global-feature extraction to better suit this challenge. 


\dc{End with a paragraph that tells how well it works...}

\matan{Are you sure we want to do that? :)}

